Playful Interactions for Representation Learning

One of the key challenges in visual imitation learning is collecting large amounts of expert demonstrations for a given task. While methods for collecting human demonstrations are becoming easier with teleoperation methods and the use of low-cost assistive tools, we often still require 100-1000 demonstrations for every task to learn a visual representation and policy. To address this, we turn to an alternate form of data that does not require task-specific demonstrations -- play. Playing is a fundamental method children use to learn a set of skills and behaviors and visual representations in early learning. Importantly, play data is diverse, task-agnostic, and relatively cheap to obtain. In this work, we propose to use playful interactions in a self-supervised manner to learn visual representations for downstream tasks. We collect 2 hours of playful data in 19 diverse environments and use self-predictive learning to extract visual representations. Given these representations, we train policies using imitation learning for two downstream tasks: Pushing and Stacking. We demonstrate that our visual representations generalize better than standard behavior cloning and can achieve similar performance with only half the number of required demonstrations. Our representations, which are trained from scratch, compare favorably against ImageNet pretrained representations. Finally, we provide an experimental analysis on the effects of different pretraining modes on downstream task learning.

==> acknowledgements.tex <==
\section{Acknowledgements:} We thank Mandi, Andrew, and Daniel for helping us collect playful interaction data. We also gratefully acknowledge the support from  The Open Philanthropy Project and Berkeley DeepDrive.

% \noindent \emph{Acknowledgements:} We thank Mandi, Andrew, and Daniel for helping us collect playful interaction data. We also gratefully acknowledge the support from  The Open Philanthropy Project and Berkeley DeepDrive.

==> old_intro.tex <==
\section{Introduction}



% — para 1 — General introduction into imitation and some problems LP: need to make it more about imitation learning rather than RL.
Imitation learning has proven to be a powerful approach to learn complex robotic skills from visual observations~\cite{zhang2018deep, stadie2017third,duan2017one,zhu2018reinforcement}. Recent works have shown how simple approaches like behavior cloning can reliably replicate desirable manipulation behaviors without needing explicit reward feedback~\cite{ho2016generative, kalashnikov2018qt,kaelbling1996reinforcement}. However, such techniques suffer from two fundamental challenges. First, compounding errors results in distribution shift~\cite{ross2011reduction} and brings the robot to parts of the state-space not supported by the expert demonstration. Second, obtaining generalizable policies requires demonstrations in a large variety of environments during training~\cite{gupta2018robot}. To tackle this problem, current methods collect large amounts of demonstrations, often in the order of 100-1000 demonstrations for a given task. The need to collect large-scale expert demonstrations is restrictive if we want our robots to solve multiple tasks. 

One path to efficient imitation learning is to use better representations. Recent work in self-supervised learning for computer vision~\cite{simclr,moco2,byol} has demonstrated how unlabeled data can be used to train powerful visual representations. In the context of imitation learning, we can use these ideas to improve the efficiency of training and learn robotic skills with fewer expert demonstrations. But how do we obtain unlabeled data for imitation? 
% — para 2 — intro to play as a way to solve problems

Current robot learning methods inspired by human learning, such as reward and imitation learning, leave out a key component of early childhood learning -- \emph{play}. Researchers have shown that play is a fundamental component in early learning~\cite{piaget2013play, cook2011science, sim2017learning,lillard2013impact,whitebread2017role}. In the context of robot learning, play data is cheap to obtain, naturally diverse, and unstructured. These qualities allow learning from play data to be a promising method to learn generalizable policies via imitation in robotics. 

\begin{figure}[]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/fig_1_new.png}

  \caption{Our method leverages less than two hours of unlabeled, diverse, and unstructured playful interaction data to learn meaningful representations for downstream manipulation tasks such as Pushing and Stacking.} 
\label{fig:teaser}
\end{figure}

% — para 3 — how we will use play + imitation
Learning from play in simulated environments has recently shown success in planning \cite{play}. In this work, we build on these ideas and focus on learning from real-world environments. Our framework for play consists of two types of data: “playful interaction data" for early learning, and expert task-demonstration data. To enable better imitation, we propose a self-supervised approach that learns a task-agnostic visual encoder from playful interaction data. Once task-agnostic representations are learned from play, we then use a small amount of task-specific expert data to learn a policy that can generalize better to unseen environments.



% — para 4 — Key algorithmic insights to get better performance + results
Our experimental setup builds on top of DemoAT~\cite{young2020visual}, a framework that can be used to collect diverse demonstrations using Assistive Tools such as reacher-grabbers~\cite{song2020grasping}. These tools are ideal for collecting play data in the wild due to its versatility and easy setup. We adapt this framework to collecting unlabeled playful interaction data by simply asking users to “do whatever they want with this tool”. With around two hours and 30,000 frames of this self-guided playful interaction data, we train a task-agnostic model using a time-contrastive method. The weights from this model then serves as the initialization for downstream behavioral cloning. 
% Rather than fine-tuning only a few linear layers~\cite{moco2, simclr,byol}, we train on the entire network when learning downstream tasks. 
% \pa{not sure how much the contrasting here matters; b/c we are doing imitation learning, they are doing classification; it also comes across as if maybe the only delta with prior work is that we train the entire network}

To experimentally study the effects of pretraining on playful interaction data, we look at two tasks: pushing, stacking, and door opening. 
% Expert demonstrations for both tasks are taken from \cite{young2020visual}. 
While fine-tuning on these tasks, we observed that continuing to update the learned representation is crucial for improved performance. We compare our method to existing baselines that use behavioral cloning with random data augmentations, and  show that our play pretraining achieves 27\% better MSE performance during test time than ImageNet~\cite{krizhevsky2012imagenet} pretraining. Interestingly, when pretrained on top of ImageNet initialization, our method achieves 39\% better performance than training the models from random initialization. 
% Lastly, we analyze the effects of unsupervised play data on task-specific downstream tasks through ablation experiments.


% small representation learning encoder to a deeper network for downstream task learning is crucial for improved performance
% — para 5 — contributions
In summary, we present three contributions in this work. First, we demonstrate that our approach of pretraining on less than 2 hours of playful interaction data can match or outperform ImageNet baselines on two different manipulation tasks: pushing and stacking. Although the use of play data has been previously explored in the context of simulated environments \cite{play}, to our knowledge this work is the first that studies the use of this play data in real-world environments. Secondly, using a time-contrastive self-supervised objective, we are able to learn a meaningful representation that can surpass current behavior cloning baselines using only a fraction of labeled data. Third, we provide an analysis of how the amount of play data affects task performance of downstream manipulation tasks. Our playful interaction data and learned models will be publicly released on our website.
% \footnote{Website:\url{sarahisyoung.github.io/pirl.html}}

% DONE \lpnote{Play data has been previously only explored in the context of simulated environments. This work is the first that studies the use of this playful data in real environments.}
% 3: playful interaction pretraining with only a small fraction of labeled data performs as well as xxx labeled data (or) playful interaction data leads to better downstream task performance [some kind of trend for more play→ better push?]



% \href{https://sarahisyoung.github.io/pirl.html}{website}.


==> pandemic_considerations.tex <==
% The CoRL 2021 organising committee and board acknowledge the challenges in producing high-quality experimental results during the social distance policies implemented in different parts of the world. Like last year, at CoRL2020, authors affected by these policies are encouraged to submit a one-page supplemental material explaining the rationale why the evaluation methodology is sufficient, how it is deficient compared to the real-world experiments, and how their method will be experimentally validated with real data.

\section{Pandemic Considerations}
Although our paper trains on real-world data from \cite{young2020visual}, we are unable to evaluate it on a real robot, and instead use the offline MSE metric. This may raise concerns that our work would not transfer to online robotic settings. We would like to stress that the offline MSE metric does correlate with better online performance on a robot, as demonstrated by the original dataset paper \cite{young2020visual}. We are cognizant of the need for real-robotic results to verify this, but unfortunately, due to the pandemic, we did not have access to a real robot to run these experiments. 

An alternative solution to running real robot experiments include running in simulation. However, transferring the representation learned on one domain (real observations) to a different one (simulation) is in itself a challenging research problem. To show that our evaluation methodology is sufficient, we have also dedicated a subsection ‘Connecting to Real Robot Results’ to address this in the paper itself. 

In summary, even without real-robot experiments, our offline MSE evaluation shows the value of playful demonstrations for representation learning and its usefulness in robotics, which is the central claim of this paper. We plan to expand upon our work and when the situation allows, experimentally validate our results with real robot experiments.

